Named Entity Recognition with stack residual LSTM and trainable bias decoding

Recurrent Neural Network models are the state-of-the-art for Named Entity Recognition (NER). We present two innovations to improve the performance of these models. The first innovation is the introduction of residual connections between the Stacked Recurrent Neural Network model to address the degradation problem of deep neural networks. The second innovation is a bias decoding mechanism that allows the trained system to adapt to non-differentiable and externally computed objectives, such as the entity-based F-measure. Our work improves the state-of-the-art results for both Spanish and English languages on the standard train/development/test split of the CoNLL 2003 Shared Task NER dataset.

==> Knowledge.tex <==
\subsection{Word embedding}

%%% What did we use for English?
English word embedding was obtained from\footnote{https://github.com/3Top/word2vec-api/blob/master/README.md}. Embedding dimension is 100 and was trained using GloVe with AdaGrad.
For the generation of the Spanish word embeddings we followed the procedure used in~\cite{lample2016neural}.
The corpus has been the Spanish Gigaword Third Edition\footnote{https://catalog.ldc.upenn.edu/ldc2011t12}.
We use an embedding dimension of 64, a minimum word frequency cutoff of 4 and a window size of 8.

\subsection{Language Modeling}

In some experiments, we used both forward and backward language models.
We used an existing model for the English forward language model. %% Quan, which one?

The English forward language model was obtained from\footnote{https://github.com/tensorflow/models/tree/master/lm\_1b} using the One billion word benchmark\footnote{https://github.com/ciprian-chelba/1-billion-word-language-modeling-benchmark}~\cite{chelba2013one} and has a perplexity of 30.
For the backward English language model and the Spanish forward and backward ones, they were generated using an LSTM based baseline\footnote{https://github.com/rafaljozefowicz/lm}~\cite{jozefowicz2016exploring}.
This code estimates a forward language model and was adapted to estimate as well a backward language model. Language models were estimated using the One billion word benchmark.
The vocabulary for the backward English model is the same as the pregerated forward model.
The perplexity for estimated backward English language model is 46.
The vocabulary for the Spanish language models has been generated using tokens with frequency $>$ 2. The perplexity for the forward and backward Spanish language models are 56 and 57 respectively.
